Automatic Configuration of Multi-Agent Model Predictive Controllers based on Semantic Graph World Models

We propose a shared semantic map architecture to construct and configure Model Predictive Controllers (MPC) dynamically, that solve navigation problems for multiple robotic agents sharing parts of the same environment. The navigation task is represented as a sequence of semantically labeled areas in the map, that must be traversed sequentially, i.e. a route. Each semantic label represents one or more constraints on the robots' motion behaviour in that area. The advantages of this approach are: (i) an MPC-based motion controller in each individual robot can be (re-)configured, at runtime, with the locally and temporally relevant parameters; (ii) the application can influence, also at runtime, the navigation behaviour of the robots, just by adapting the semantic labels; and (iii) the robots can reason about their need for coordination, through analyzing over which horizon in time and space their routes overlap. The paper provides simulations of various representative situations, showing that the approach of runtime configuration of the MPC drastically decreases computation time, while retaining task execution performance similar to an approach in which each robot always includes all other robots in its MPC computations.

==> chapters/ParkingLot/03_method.tex <==
\section{Method}

This section is structured as follows, first, the semantic map primitives are introduced. Secondly, the proposed algorithms for the retrieval and configuration of the motion controllers of individual agents and flocks of agents are presented. Finally, the MPC formulation of the motion controllers is discussed.

\subsection{Semantic Map Primitives}
The semantic map is a graph world model that describes the environment in which the agent is deployed at the topological level. Knowledge of the geometry of the environment is represented as a property of the nodes composing the graph. In this work, we assume each agent has access to the an identical world model which contains correct information. We also assume that agents have the ability to recognize new or moved obstacles and are able to update the world model accordingly.
A simple example environment, with corresponding graph world model, is depicted in Figure \ref{fig:semi_struc_graph}. The nodes of the graph world model represent semantic elements of the environment which we refer to as semantic map primitives.  Within the context of this paper four semantic primitives are identified:  Areas, Interfaces, Walls, and Virtual Walls. 
\textbf{Areas} represent the drivable space for the agent, and are, therefore, the building blocks of the semantic plan of each agent. \textbf{Interfaces} model the connections between areas, i.e. areas are not directly connected through an edge but always through one interface node between them. Apart from connectivity, interfaces provide information on the objectives and events that influence the behavior of an agent while it is travelling between the two areas. The objectives can be seen as a measure of progress and the direction in which progress can be made. Events encode the moment the end of a certain area has been reached. Interfaces that are currently inactive for an agent, are considered to be \textbf{Virtual walls}. These virtual walls constrain the agent's behavior. The navigation through an area is furthermore constrained through the definition of \textbf{Walls}. These can stem from actual walls or obstacles in the environment, or can be defined virtually to prevent the agents from entering certain regions in its workspace. To enable safe navigation through areas these are considered hard constraints on the agent's movement. 
The semantic maps are represented in a graph database, the 2D geometric information of elements is encoded as lines and polygons. The definition of a graph world model allows us to name relations between entities, and to query these named relationship. This, for instance, allows for the retrieval of all walls, and their geometry, which are related to a certain named area.  
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.4\linewidth}
    \resizebox{\linewidth}{!}{\input{Figures/simple_example_sketch.tex}}
    \caption{}
    \label{fig:semi_struc_env}
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.45\linewidth}
    \resizebox{\linewidth}{!}{\input{Figures/simple_graph_sketch}}
    \caption{}
    \label{fig:semi_struc_graph}
    \end{subfigure}
    \caption{(Left) Simplified semi-structured environment consisting of three areas. (Right) Excerpt of a graph world model describing the environment on the left.}
\end{figure}

\subsection{Navigation Strategy}

Commonly used navigation approaches often specify the task description of a navigation task either as tracking a pre-specified path or trajectory, or as reaching a certain final pose \cite{}. In this work we take a different approach. We decompose the task of reaching a certain final position into sub-tasks, which we specify as a sequence of areas (a route) to be traversed. The agents need to travel along this route towards their goal while avoiding collisions with walls or other agents. The advantages of this approach are ....
\todo[inline]{Cesars input: Integrated planning and control. Taking into account kinematic constraints at all level. Smoother control actions. Planning at necessary resolution. Coarse planning, more compatible with topological planning, more scalable. Included above not happy yet.}
For example, consider again the environment depicted in Figure \ref{fig:semi_struc_graph}, and an agent located in Area $S_0$. Instead of formulating the navigation task as reaching a certain coordinate, the navigation task can be formulated by specifying the route, in this case, the task specification is \lq\lq\textit{reach $I_3$ after crossing areas $S_0$, $S_1$ and $S_2$}\rq\rq. 
Specifying the local navigation tasks as a route, combined with the graph world model in Figure~\ref{fig:semi_struc_env}, allows the agent to reason about which elements in the world are relevant for the currently active sub-task, e.g. walls or agents which are only linked to topologically far-away areas are not relevant at this time instance, which reduces the complexity of the navigation problem.
%
\todo[inline]{NOTE ELENA: We need to specify the graph world model formally}
%
Given the graph world model in definition \ref{empty_ref}, the multi-agent navigation problem can be specified as, consider a team of $N_A$ agents that is deployed in an environment of which a graph world model that follows the definition in \ref{empty_ref} is available.
Agent $A_i$ is tasked with moving from its current position $\vx_{i,0}$ in area $S_{i,0}$ to its goal area $S_{i,g}$. A route $\vP_i = [S_{i,0} \dots S_{i,g}]$ to complete its task is provided to the agent, e.g. by a fleet-management system. It is assumed that, under nominal undisturbed conditions, execution of plan $\vP_i$ leads to a successful completion of the task, i.e. that both task and plan are feasible. The task is deemed to be successfully completed once agent $A_i$ is contained within area $S_{i,g}$ without having collided with any other agent $A_j$ or with any element of the environment. Within our approach, we define the \text{modes} $\vm$ of the agents $\mathbb{A}$ as the index in the plan corresponding to the area an agent is currently contained in. Within mode $m_i$ the objective of agent $A_i$ is the objective encoded by the interface that connects areas $S_{i,m_i}$ and $S_{i,m_{i+1}}$. The set of hard environmental constraints $\mathbb{W}_i$ to which the agent $A_i$ is subjected contains only those (virtual-)boundaries which are connected via vertices to the current area. The inter-agents constraints are formulated between couples of agents $c_i := (A_i, A_j)$ which are traversing in the same area.  Once the agent reaches the currently active interface, the mode variable is incremented, and the objective and constraints are updated. 
To decrease the influence of discrete transitions between areas $S_{i,m_i}$ and $S_{i,m_{i+1}}$, a semantic horizon $\vh$ is introduced, which acts as a look ahead on the objectives and constraints of the next $N_{h}$ areas in the pre-specified planning. It effectively means, that not only does the agent take into account elements and agents in the current area $S_{i,m_i}$, but it, furthermore, takes into account any element or agent in any area $S_{i,h}$, with $h$ being any area which is contained within both the agent's plan and semantic horizon. Figure \ref{fig:semhorizon} depicts the semantic horizon, and corresponding constraints, for an example scenario. The algorithm for retrieving relevant elements and the algorithm for retrieving the relevant agent configuration, given the graph world model $K$, are reported on in more detail in algorithms \ref{alg:rel_el} and \ref{alg:rel_ag} respectively.
%
\begin{figure}[t]
    \centering
    \resizebox{0.5 \linewidth}{!}{\input{Figures/semantic_horizon}}
    \caption{Illustration of two agents with overlapping semantic horizons with $N_{h} = 2$. Red and blue polygons illustrate the  wall constraints of the red and blue agent respectively. Purple polygons show the overlap between the two. Dashed lines illustrate the virtual wall constraints. }
    \label{fig:semhorizon}
\end{figure}

\begin{algorithm}[ht!]
    \caption{Relevant element retrieval for agent $A_i$}\label{alg:rel_el}
    \begin{algorithmic}
    \State \textbf{Input:} $K$, $\mathbb{P}_i$, $m_i$, $N_{h}$
    \For{ $j \gets m_i$ to $m_i + N_{h}$  }
        \State $\mathbb{W}_{i,j} \gets \text{walls from } $K$ \text{ related to } \mathbb{P}_i [j] $
        \State $\mathbb{V}_{i,j} \gets \text{interfaces from } $K$ \text{ related to } \mathbb{P}_i [j] \land \neg \mathbb{P}_i [j \pm 1]$
        \State $\mathbb{I}_{i,j} \gets \text{interfaces from } $K$ \text{ related to } \mathbb{P}_i [j] \land \mathbb{P}_i [j + 1]$
        \State $\mathbb{O}_{i,j} \gets \text{objectives from } $K$ \text{  related to } \mathbb{I}_{i,j}$
        \State $\mathbb{E}_{i,j} \gets \text{events from } $K$ \text{ related to } \mathbb{I}_{i,j}$
    \EndFor
    \State \textbf{Return:} $\mathbb{W}_i$, $\mathbb{I}_i$, $\mathbb{O}_i$, $\mathbb{E}_i$
    \end{algorithmic}
\end{algorithm}
%
\begin{algorithm}[ht!]
    \caption{Relevant agent configuration retrieval}\label{alg:rel_ag}
    \begin{algorithmic}
        \State \textbf{Input:} $K$, $\mathbb{A}$, $\mathbb{P}$, $\vm$, $N_{sh}$
        \State $c \gets \emptyset$, \hspace{0.25 em} $\mathbb{A}_f \gets \emptyset$
        \State \textbf{\textit{Find couples of agents which have overlap}}
        \For{ $i \gets 0$ to $N_{A}$}
            \State $\vh_i \gets \mathbb{P}_i[m_i:m_i + N_{h}]$
            \For{$j \gets i+1$ to $N_{A}$}
                \State $\vh_j \gets \mathbb{P}_j[m_j:m_j + N_{h}]$
                \If{$\vh_i \cap \vh_j \neq \emptyset$}
                    \State $c \gets c \cup \{(A_i, A_j)\}$
                    \State $\mathbb{A}_f \gets \mathbb{A}_f \cup \{A_i\} \cup \{A_j\}$
                \EndIf
            \EndFor
        \EndFor
        \State \textbf{\textit{Expand flocks}}

        \State $\mathbb{F}^k  \gets c$ \Comment{Flocks at iteration 0}
        \While{$ \mathbb{F}^k \neq \mathbb{F}^{k+1} $}
        \State $\mathbb{F}^{k+1} \gets \emptyset$
        \For{$\mathbb{F}_i \text{ in } \mathbb{F}^k$}
            \For{$\mathbb{F}_j \text{ in } \mathbb{F}^{k+1}$}
                \If{ $\mathbb{F}_i \cap \mathbb{F}_j \neq \emptyset$ }
                    \State $\mathbb{F}_i \gets \mathbb{F}_i \cup \mathbb{F}_j$
                \EndIf
            \EndFor
            \State $\mathbb{F}^{k+1} \gets \mathbb{F}^{k+1} \cup \{\mathbb{F}_i\}$
        \EndFor
        \EndWhile
        \State \textbf{\textit{Add agents without overlap}}
        \State $\mathbb{F} \gets \mathbb{F} \cup ( \mathbb{A} \setminus \mathbb{A}_f)$
        \State \textbf{Return:} $\mathbb{F}$ \Comment{Flocks: Set of sets of relevant agents}
        \end{algorithmic}
\end{algorithm}
%
\subsection{MPC Formulation}
% i,j agent
% k time step
% l agent mode
% m element counter 
% t absolute time
The local navigation problem, formulated using the algorithm as it has been formulated so far, is solved using a Model Predictive Control (MPC) approach. For each set of relevant agents, i.e. flock,  $\mathbb{F}_o \in \mathbb{F}$, a set of relevant Objectives $\mathbb{O}_i$, and a set of relevant environment elements and virtual elements $\mathbb{W}_i$ for each $A_i \in \mathbb{F}_o$ the centralized multi-agent MPC problem can be formulated, for each flock, as:
\begin{align}
    &\min_{\vx, \vu} \sum_{i = 0}^{|\mathbb{F}_o|} J_i(\vx_i, \vu_i, m_i, t), \\
    \text{s.t.} \quad  &\vx_i(t + k + 1) = \vf_i (\vx_i(t + k), \vu_i(t + k)),\\
    &\vx_i(t) = \vx_{i, init},\\
    & \vx_{i,min} \leq \vx_i(t + k) \leq \vx_{i,max},\\
    & \vu_{i,min} \leq \vu_i(t + k) \leq \vu_{i,max},\\
    &\text{dist}\left(A_i\left(t + k\right), w\right) \geq 0, \quad  \forall w \in \mathbb{W}_i, \\
    &\text{dist}\left(A_i\left(t + k\right), A_j\left(t + k\right)\right) \geq 0,\quad \forall A_j \in \mathbb{F}_j \land j\neq i,
\end{align}
in which $\vf_i$ describes the dynamic model of agent $i$, which within the context of this paper is assumed to reflect a kinematic unicycle model. Furthermore, $\vx_i \in \mathbb{X}_i$ and $\vu_i \in \mathbb{U}_i$ represent the state and input of agent $i$ respectively. The state of agent $i$ describes its longitudinal velocity and its Cartesian position and orientation w.r.t a global reference frame. The control input of agent $i$ are the acceleration in longitudinal direction and its angular velocity.

%\todo[inline]{Overlap in indices between $\mathbb{F}_i$ and $A_i$}
\subsubsection*{Objective}

Within the MPC formulation we employ a standard cost function structure, containing intermediate costs $l_i$ and final costs $n_i$,
\begin{align}
    J_i(\vx_i, \vu_i, m_i, t) := \sum_{k = 0}^{N_t} &l_i(\vx_i(t + k), \vu_i(t+k))\\
    &+ n_i(\vx_i(t + k), m_i),
\end{align}
with $\vx_i \in \mathbb{X}_i$ and $\vu_i \in \mathbb{U}_i$ the state and inputs of agent i respectively, $t$ the current time step, $N_t \in \mathbb{N}$ the prediction horizon, and $m_i \in \mathbb{N}$ the mode of the system which arises from the decomposition of the navigation task into subtasks.
Within the context of this paper the intermediate cost function is defined as
\begin{equation}
    l_i(\vx_i,\vu_i,t) := \vu_i^T \vR_i \vu_i,
\end{equation}
with $\vR_i$ a cost matrix of appropriate dimension that weights the system input of agent $i$. The terminal cost function rewards progress made within the prediction horizon and is thus defined as
\begin{align}
    n_i(\vx_i, t, m_i) &:= \sum_{j=0}^{N_{h}} w_o(\vx) \ d_{i,j}^T \ \vQ_{i,j} \ d_{i,j}, %\\
             %&\phantom{:}= \vx^T \vA^T \vQ \vA \vx + 2 \vB^T \vQ \vA x + \vB^T \vQ \vB
\end{align}
with $d_{i,j}$ the (signed) distance of agent $A_i$ from the $j-th$ element of the set of active objectives $\mathbb{O}_j$, with $w_o$ weighing the objectives according to the progress made so far.  
%\todo[inline]{Do we need to be more specific on the determination of the weights. They are determined based on the mode of the end of the prediction horizon}
% \begin{equation}
%     d_i(\vx, t):=  \vA_i(l_i) \vx_i(t) + \vb(l_i)
% \end{equation}

% \begin{align}
%     \vA_i(l_i) &:=
%     \begin{bmatrix}
%         a^{*}, b^{*}
%     \end{bmatrix},&
%     \vb_i(l_i) &:= c^*
% \end{align}


% \begin{equation}
%     p^* := \frac{p}{\sqrt{a^2 + b^2}}
% \end{equation}


\subsubsection*{Constraints}
For the safety of the agents and the environment, agents should not collide with any elements, e.g. walls, obstacles, virtually defined boundaries, in the environment, nor with each other. To represent the no-collision constraints we make use of the separating hyperplane constraint formulation as it has been described in~\cite{OMGtools2016}. The formulation allows the specification of no-collision constraints between agents and obstacles described by convex shapes, however, puts no limitation on the convexity of the resulting drivable space. This opposed to, for example, making use of linear constraints which only allows for describing a convex drivable space.

For each element $w \in \mathbb{W}_i$ with vertices $\vv_{w}$, we formulate the no-collision constraints for a circular~agent $A_i$ with radius~$r_v$~as:
\begin{align}
    \va_{w,i}^T \vv_{w,j}- \vb_{w,i} &\geq 0,   &&\forall \vv_{w,j} \in \vv_w,\\
    \va_{w,i}^T \vx(k) - \vb_{o,i} &\leq -r_v,  &&\forall k \in [0,N_t],\\
    ||\va_{w,i}||_2 &\leq 1,
\end{align}
with $\va$ and $\vb$ the normal vector to and offset of the hyperplane respectively. Since we consider circular agents, the no-collision constraint between any two agents $i$ and $j$, with radii $r_i$ and $r_j$ respectively, can be formulated as
\begin{align}
    || \vx_{k,i} - \vx_{k,j} ||_2 &\leq (r_i + r_j), &\forall k &\in [0, N_t].
\end{align}
To encourage trajectories further away from constraints, all no-collision constraints are augmented with soft constraints.


==> chapters/ParkingLot/04_results.tex <==
\section{Validation}

\subsection{Implementation}

The algorithm described in the paper, along with an example simulation environment has been made available \footnote{Code is available at: } %\url{https://gitlab.tue.nl/s154460/Semantic_MPC_Configuration}}. 
The algorithm was implemented in Python, with the MPC controller implemented using the do-mpc package \cite{DOMPC2017}. The resulting optimization problem is solved using CasADi \cite{CasADi2019} and the HSL\_MA27 \cite{HSL} solver in IPOPT\footnote{The max\_iter parameter of IPOPT is set to $150$ [-], max\_cpu\_time is set to $0.5 \ [s]$.} \cite{wachter2006implementation}. The graph querying is implemented in SPARQL using the RDFLib package \cite{RDFLib}. Simulations are implemented using the built-in simulation in do-mpc, as well as in PyBullet \cite{coumans2021}. Validation results\footnote{Results were obtained on an Intel Core i5 13500 processor running Ubuntu 20.04 under Windows Subsystem for Linux 2 (WSL2)} are obtained from the built-in simulation unless explicitly mentioned.
%\todo[inline]{Scenario results are done using simple simulation because of long simulation times in PyBullet (since it is real time).}

\subsection{Simulation Environment}
To validate the method, a simulation environment was designed in which multiple agents could be deployed. The environment is depicted in Figure \ref{fig:simenvscenarios}. The environment workspace is approximately $20 \text{ by } 23 \ [m]$ in size. The corridor width of each corridor is approximately $2.0 \ [m]$. The velocity of each agent is limited to the range $[0, \ 1.0] [m/s]$, their longitudinal acceleration and angular velocity to $[-0.25, \ 0.25] [m/s^2]$ and $[-0.5, \ 0.5] [rad/s]$ respectively. The time step of the MPC controller is $0.5 \ [s]$. The length of the prediction horizon is equal to 25 time steps. During each simulation run a set of agents is deployed within the area, tasked with reaching their respective goal areas after crossing a pre-specified sequence of areas.
During the experiments it is assumed that agents are homogeneous, more specifically all agents can be contained in a cylinder with a base raidus of  $0.3 \ [m]$. Dynamically agents are described by a kinematic unicycle model. Simulations are performed for a dynamic flock formation case, in which the set of agents communicating and cooperating is dynamically determined, for a case in which agents are always part of the same flock, and for a case in which agents do not cooperate. 

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[c]{0.6\linewidth}
%     \resizebox{\linewidth}{!}{\input{Figures/example3}}
%     \end{subfigure}
%     \caption{Drawing of the simulation environment in which the agents are deployed. Area names are written in their respective areas. Drivable space is denoted in gray.}
%     \label{fig:simenv}
% \end{figure}


\subsection{Tested Scenarios}
In order to validate the method we introduce four distinct scenarios. In each of the four scenarios, a number of robotic agents is tasked with completing the route, a sequence of areas to be traversed, they receive at the start of the simulation. The difference between scenarios is mainly the amount of agents in the environment, and the expected amount of interaction required to complete the pre-specified plan, i.e. the amount of overlap in the plans. For each scenario a number of different starting areas and corresponding plans are introduced, each starting area and corresponding plans is referred to as a sub-scenario.
The individual scenarios are depicted in Figure \ref{fig:simenvscenarios}.
In scenario A, two agents are deployed within the environment. Their plans do not overlap. In scenario B, similar to scenario A, two agents are deployed, but their plans show partial overlap. Scenario C involves four agents with partially overlapping plans. The agents have overlap in plans, but the maximum number of agents at each overlap is limited.  Finally, in scenario D, four agents arrive at a crossing at the same time, the maximum overlap involves four agents.
\begin{figure*}[t]
    \centering
    \begin{subfigure}[c]{0.2\linewidth}
    \resizebox{\linewidth}{!}{\input{Figures/scenarioA.tex}}
    \subcaption*{A}
    \end{subfigure}
    ~
    \begin{subfigure}[c]{0.2\linewidth}
        \resizebox{\linewidth}{!}{\input{Figures/scenarioB.tex}}
        \subcaption*{B}
    \end{subfigure}
    ~
    \begin{subfigure}[c]{0.2\linewidth}
        \resizebox{\linewidth}{!}{\input{Figures/scenarioC.tex}}
        \subcaption*{C}
    \end{subfigure}
    ~
    \begin{subfigure}[c]{0.2\linewidth}
        \resizebox{\linewidth}{!}{\input{Figures/scenarioD.tex}}
        \subcaption*{D}
    \end{subfigure}
    \caption{Sub-scenarios of scenarios A,~B,~C and~D respectively. Agents are initialized in the darkest shade of their respective color, and are tasked with navigating through the lighter shades. Note the overlapping colors in scenarios B,~C and~D. Overlaid are the resulting trajectories of one of the runs of the dynamic cooperation case.}
    \label{fig:simenvscenarios}
\end{figure*}


% \textbf{Two agents far apart from each other. Plans don't overlap.}

% \textbf{Two agents start far apart from each other. Plans do overlap.}

% \textbf{Four agents start far apart from each other. Plans do overlap, but not at the same time.}

% \textbf{Four agents start at common intersection, navigate away from it.}

\subsection{Metrics}
The behavior of the algorithm in the scenarios will be evaluated by introducing metrics that enable the comparison of the behavior of the agents when using dynamic flock formation, when agents always cooperate, and when agents do not cooperate at all. Results from each sub-scenario will be averaged over a set of separate runs of that scenario. In each run, a random feasible initial pose is generated within the start area of each agent's plan.
The first metric to be analyzed, is the task completion time of each agent. This time is computed as the time it takes for the last agent in each run to reach their final mode. We report the minimum, maximum and average over all runs of each scenario for the \textit{dynamic cooperation} and \textit{always cooperate} cases relative to the completion time of the non-cooperating agents.
% Secondly, we report on the shortest distance from the static elements in the environment:
% \begin{equation}
%     d_{o} := \min_t \left[ dist(\vx_i(t), \vo) \right] - r_i \qquad \forall i \in \mathbb{A} \land \forall \vw \in \mathbb{W}
% \end{equation}
% in which $\vx_i(t)$ the state of agent $i$ at time $t$, $\vo$ the obstacle position, and $r_i$ the radius of agent $i$. Furthermore, we report the minimum distance to other agents.
% \begin{equation}
%     d_{A} := \min_t \left[ dist(\vx_i(t), \vx_j(t)) \right] - r_i - r_j \qquad \forall i,j \in \mathbb{A} \land i \neq j
% \end{equation}
% These metrics are used as a measure for the reliance on accurate localization and as a robustness against unknown disturbances. We again report on the minimum, maximum and average over all variations of each scenario.
Lastly we report on the time it takes to compute a solution, and the correctness and feasibility of these solutions. In the case of computation time, we report both on solver time, and configuration time, the latter including the time required to query the graph world model and set up the MPC problem. For each time step the maximum time is taken over all currently active solver instances, since each solver can be executed in parallel. We again report the minimum, maximum and average over all runs of each scenario. Collisions and infeasibilities are reported on through the number of runs in which they occur.
%\todo[inline]{Explain why we take the maximum per time iteration, parallel}

\subsection{Results}
For visualization purposes, an example realization of a run of the dynamic cooperation case of each scenario has been overlaid in Figure \ref{fig:simenvscenarios}. The remaining of this section will present the results of the earlier introduced metrics.

\subsubsection{Completion}
For each sub-scenario Table \ref{tab:success} summarizes the number of non-successful task completions for each flock formation case. It is observed that in scenario A all cases lead to successful task completion, except for one in both the never and dynamic flock formation cases, which were both due to infeasibility in one of the runs. 
In scenario B and C, the majority of never cooperate runs fail due to collisions. This is expected due to the lack of collision constraints between agents when there is no cooperation. The always and dynamic cases fail due to the detection of infeasibilities, and due to minor collisions. The latter only occurring in between sample points and thus not triggering an infeasibility.
From Table \ref{tab:success} it is apparent that scenario D is the most challenging even in the always and dynamic flock formation cases. In both cases eight out of 51 cases fail due to minor collisions in between sample points, one fails due to an in feasibility. The never cooperate case fails due to collisions between agents, again due to the lack of no collision constraints.
\subsubsection{Completion Time}
The time it takes, measured in amount of time steps, for all agents to finish their task in the given scenario is reported on in Table \ref{tab:tcomplete}. It is apparent, from the average relative completion time, that the results obtained in the Always and Dynamic cases are largely comparable to each other. The never cooperate case does perform better, leading to shorter completion, however, this approach leads to the highest number of observed collision, which can both be explained by the lack of no-collision constraints in the MPC formulation in this case allowing for trajectories that do intersect each-other.
\begin{table}[]
    \centering
    \caption{Non-successful Completion of each sub-scenario for the \textbf{A}lways, \textbf{D}ynamic and \textbf{N}ever flock cases, due to infeasibilities/ collisions.}
    \begin{tabular}{cc|ccc}
         & N & \textbf{A} & \textbf{D} & \textbf{N} \\
         &   & infeas. / coll. & infeas. / coll. & infeas. / coll.\\
         \hline
    A              &    52                & 0 / 0     & 1 / 0      & 1 / 0      \\
    B              &    52                & 2 / 0     & 1 / 0      & 1 / 26        \\
    C              &    52                & 0 / 1     & 0 / 0      & 0 / 52         \\
    D              &    51                & 1 / 8     & 1 / 8      & 1 / 50            \\
\end{tabular}
\label{tab:success}
\end{table}

\begin{table}[]
    \centering
    \caption{Comparative completion time, in time steps, of completed runs for the \textbf{A}lways, \textbf{D}ynamic and \textbf{N}ever flock cases. [minimum, average, maximum] of always and dynamic cases are reported w.r.t the never case results.}
    \begin{tabular}{c|cc|c}
    $T_{task}$     & \textbf{A w.r.t N} & \textbf{D w.r.t N} & \textbf{N} \\ 
         & [min, avg, max] & [min, avg, max]& [min, avg, max]\\
         \hline
    A                                  & {[}0.70, 0.99, 1.11{]}  &  {[}1.00, 1.00, 1.00{]}    & {[}56, 95 ,138{]}        \\
    B                                  &  {[}0.90, 1.10 ,1.67{]} &  {[}0.92, 1.04 ,1.27{]}      & {[}76, 101 ,135{]}      \\
    C                                  & {[}0.70, 1.08, 1.61{]} & {[}0.85, 1.03, 1.45{]}       & {[}72, 108, 150{]}         \\
    D                                  & {[}0.79, 1.25, 2.55{]} &  {[}0.79, 1.18, 1.98{]}                       & {[}70, 102, 157{]}                      \\
\end{tabular}
\label{tab:tcomplete}
\end{table}

\subsubsection{Computation Time}

The MPC computation times obtained from the simulations are reported on in Table \ref{tab:tmpc}. The average number of flocks and thus MPC controllers, and the average number of agents within a flock, are reported on in Table \ref{tab:flocksize}. From Table \ref{tab:tmpc} it is observed that the MPC computation times of the Dynamic case are, on average, lower than the always cooperate case, but higher than the never cooperate case. In scenario A, no plan overlap occurs, which leads to the Dynamic case performing, on average, the same as the never case. In scenario D, four agents arrive at the same intersection leading to the method performing more similar, but still better, to the always case. The computation and MPC configuration time, are plotted in Figure \ref{fig:tmpc_comparison} for an agent during ten different runs of sub-scenario B.0 in Figure \ref{fig:simenvscenarios}. The figure shows that, for the dynamic cooperation case, at the start of the plan execution the agents have non-conflicting semantic horizons. After some time their horizons start to overlap, leading to higher computation times. Once the agents leaves the semantic horizon of the other, computation times reduce to the level of the never cooperate case. From the figure it is also apparent that relatively high computation and configuration times occur after each mode switch of the agent. These relatively high computation times partially explain the relatively low minimum and high maximum values in Table \ref{tab:tmpc}, which occur when there are small mismatches in switching times between the never and always or dynamic cases.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1\linewidth]{Figures/t_mpc_comp.pdf}
%     \caption{The computation and configuration times for an agent in ten different runs of scenario B.0 for the \textbf{A}lways, \textbf{D}ynamic and \textbf{N}ever flock formation cases. Each color represents a separate run.}
%     \label{fig:tmpc_comparison}
% \end{figure}

\begin{table}[t]
    \centering
    \caption{Comparative computation time of completed runs for the \textbf{A}lways, \textbf{D}ynamic and \textbf{N}ever flock cases. [minimum, average, maximum] of always and dynamic cases are reported w.r.t the never case results.}
    \begin{tabular}{c|cc|c}
    $T_{mpc}$     & \textbf{A w.r.t N} & \textbf{D w.r.t N} & \textbf{N} \\ 
         & [min, avg, max] [-]& [min, avg, max] [-] & [min, avg, max] [s] \\
         \hline
    A                                  & {[}0.41, 2.37, 14.0{]}  &  {[}0.53, 1.00, 1.28{]}    & {[}0.02, 0.04, 0.24{]}        \\
    B                                  &  {[}0.53, 2.29, 9.75{]} &  {[}0.32, 1.50, 6.65{]}      & {[}0.02, 0.04, 0.22{]}      \\
    C                                  & {[}1.07, 6.16, 26.1{]} & {[}0.38, 2.24, 15.7{]}       & {[}0.03, 0.05, 0.26{]}         \\
     D                                  & {[}1.24, 5.96, 31.2{]} &  {[}0.31, 3.95, 30.2{]}                       & {[}0.03, 0.05, 0.23{]}                      \\
\end{tabular}
\label{tab:tmpc}
\end{table}

\begin{table}[t]
    \centering
    \caption{Average number of flocks/average size of flocks for the \textbf{A}lways, \textbf{D}ynamic and \textbf{N}ever flock cases.}
    \begin{tabular}{c|ccc}
      $\mathbb{F}$   & \textbf{A} & \textbf{D} & \textbf{N} \\
         & avg nr. / avg size & avg nr. / avg size & avg nr. / avg size
         \\ \hline
    A              & 1.0 / 2.0     & 2.0 / 1.0   &  2.0 / 1.0     \\
    B              & 1.0 / 2.0     & 1.6 / 1.4   &  2.0 / 1.0        \\
    C              & 1.0 / 4.0     & 3.0 / 1.5   &  4.0 / 1.0         \\
    D              & 1.0 / 4.0     & 2.5 / 2.2   &  4.0 / 1.0            \\
\end{tabular}
\label{tab:flocksize}
\end{table}

==> chapters/ParkingLot/Introduction.tex <==
Our contribution is twofold.
Firstly we propose a semantic graph world model that captures both the topology and the geometry of the environment in the form of a property graph. The topology of the graph is designed to allow agents to dynamically and automatically derive which constraints and objective functions are applicable to their MPC controller given the current state of the system as represented in the graph.  Secondly, we propose an algorithm to dynamically determine which agents should coordinate their movements which results in a reduction of the number of contraints in the MPC controller of each agent which result in a significant reduction in communication and computation time of the MPC controller. 

Our contribution is threefold.
Firstly we introduce a semantic world model that captures both the topology and the geometry of the environment in the form of a property graph. These world models are tailored to allow agents to configure their (model predictive) controllers for a local navigation task in these environments. Secondly we propose an algorithm to dynamically determine which agents should coordinate their movements, based on their current plan and the semantic description of the environment. We show that, through the use of this dynamic cooperation approach, a reduction in MPC computation time can be achieved in certain scenarios when compared to an approach in which cooperation is always enabled. Finally, we present an MPC formulation that is tailored to allow the inclusion of constraints based on their relevance according to the above algorithms. 


==> chapters/ParkingLot/RelatedWork.tex <==
such as planning (
% Classical multi-agent navigation approaches include reactive methods like: the dynamic window approach \cite{580977}, velocity obstacles \cite{fiorini1998motion}, reciprocal velocity obstacles \cite{4543489}, and artificial potential fields \cite{1285656}. Generally, the disadvantages of reactive methods include that in dense dynamic environments the resulting robot behavior tends to result in short-sighted and oscillatory
% behavior, due to their one step ahead planning approach. Furthermore, they cannot guarantee task completion, nor that they are deadlock free \cite{7138650}.
% In planning approaches, a multi-robot planner computes conflict-free trajectories that lead all robots from the start to a goal position. Coupled approaches, in which the trajectories of robots are planned jointly, come with a high computational complexity, and often require robots to execute the plan exactly as prescribed which is an issue in structured environments with dynamic obstacles which are difficult to exactly model or predict. Decoupled approaches, such as prioritized planning, plans are computed independently or sequentially suffer from incompleteness \cite{7138650}. 

Several approaches have been proposed to address multi-agent navigation problems.  In planning approaches (e.g., \cite{standley2011complete,WAGNER20151, standley2011complete, 7138650}), a multi-robot planner computes conflict-free trajectories for each robot. Coupled approaches (e.g., \cite{standley2011complete,WAGNER20151}), in which the trajectories of robots are planned jointly, come with a high computational complexity. In decoupled approaches \cite{velagapudi2010decentralized,7138650}, such as prioritized planning, plans are computed independently or sequentially. Decoupled approaches tend to suffer from incompleteness, especially in dense environments~\cite{7138650}. Planning approaches, furthermore, often require robots to execute the plan exactly as prescribed which is an issue when dynamic obstacles are present. \newline
Reactive methods to address multi-robot navigation include the dynamic window approach \cite{580977}, velocity obstacles \cite{fiorini1998motion}, reciprocal velocity obstacles \cite{4543489}, and artificial potential fields \cite{1285656}. Due to their one-step ahead approach, reactive methods tend to be challenged in dense dynamic environments resulting in short-sighted and oscillatory behavior. Furthermore, they usually do not provide guarantees on task completion or deadlock freeness \cite{7138650}. %
%
% In prioritized planning approaches, a subset of decoupled approaches, robot trajectories are planned one after another based on their unique priority~\cite{7138650}.
%
%
% % Scheduling (especially at intersections)
% Scheduling:
% \cite{colombo2014least}
% \cite{7823100}
% \cite{6495719}
%
% % Prio
% Prioritization: \cite{7138650}\\
% % Reactive methods
% DWA: \cite{580977}\\
% velocity obstacles: \cite{fiorini1998motion}\\
% RVO: \cite{4543489}\\
% BVD: \cite{7828016}\\
% APF: \cite{5152765} \cite{1285656}\\
%
% This one
%\cite{patwardhan2022distributing}
%
% Cell discretization
% The authors of \cite{ROSZKOWSKA202287} propose a framework in which 
% collision-free navigation is achieved through a cell decomposition of the environment. Separate levels of the framework are responsible for the allocation of agents to cells, and the coordination within cells.
%
% the multi-agent coordination problem is split into three levels. A Discrete Event System based cell transition controller ensures that the allocation of agents to each of the cells, in which the environment is divided. The cell traverse controller, based on either roundabout behavior or Artificial Potential Fields (APF), is responsible for the collision-free motion of agents within a cell. The lowest level is responsible for the continuous-time robot control.
%

A framework which is able to consider longer prediction horizons, and able to explicitly take into account hard constraints, such as no-collision constraints, is Model Predictive Control (MPC). In MPC-based approaches, trajectories are computed by solving a constrained optimization problem. The objective function is commonly a measure of the desired performance of the system. Constraints typically arise from the system dynamics, hardware limits, and (safety-) requirements. Within the context of mobile-robot navigation, different MPC formulations has been proposed, e.g.,  \cite{mercy2018online, ferranti2018coordination, 9981780}. Similarly to the scenarios addressed by this work,  \cite{mercy2018online} consider robot navigation in environments with an inherent structure. They introduce the use of   separating hyperplane constraints for collision avoidance which this paper adopts in the proposed MPC formulation as well.
%
On the same line but for vessels navigation, \cite{ferranti2018coordination}, designed a distributed nonlinear MPC for the navigation of vessels at a canal intersection. 
%
In \cite{9981780} a framework is described to tune the MPC controller of an autonomous racecar based on the current environmental conditions using a Bayesian optimisation approach.  

MPC approaches, however, often suffer from issues with scalibility as the number of agents grows large \cite{firoozi2020distributed}. To address the scalability many authors have proposed decentralizing the MPC problem \cite{ferranti2018coordination,serra2020whom, mercy2018online}. This, however, often comes at the cost of an increased need for communication due to the coupling between sub-problems resulting from agents sharing the same workspace.
%
Several works have proposed reducing the complexity of the MPC problem itself. The proposed methods typically use the current context to reduce the number of optimisation variables and/or constraints, or to decouple problems which are unlikely to influence each other. The authors of \cite{serra2020whom} propose a framework in which a multi-agent MPC trajectory planner is deployed alongside a communication policy that, using a multi-agent reinforcement learning approach, has learned when and with whom the agent should communicate to avoid collisions in an empty world.
%The resulting agents show similar behavior to a broadcasting approach, while significantly reducing communication needs. They, furthermore, show improved performance over distance-based heuristic approaches. 
The authors of \cite{mercy2018online} combine a global path planner with a local trajectory generator. This approach allows them to divide the task of navigating a large and complex environment into smaller frames, reducing the scope and complexity of subsequent optimal control problems.

%\cite{9981780}


% In \cite{ROSZKOWSKA202287}, the responsibilities for coordination are split among levels. Reasoning for the need of coordination is done through the use of a cell decomposition. The highest level coordinates the presence of agents in cells. The coordination on a continuous-state level is done among all agents in a cell.

%% Add some of the other approaches

% \subsection{The use of knowledge graphs in a (multi-)robotic context}
% Our paper is not the first to propose algorithm that exploit prior knowledge, encoded as knowledge graphs, in a \mbox{(multi-)robot} context. In \cite{pauwels2023live} knowledge graphs are generated from existing Building Information Models. The knowledge graphs as a database in which features are stored for a 2D localization approach
% \cite{9561129}. 

% \todo[inline]{Little actual application in the below}
% The authors of \cite{el2020aware} propose an ontology, a reasoner, and a set of behavioral rules. The behavioral rules are analogues to behavioral rules, and combined with the robot's perception are the basis of the robot's policy.    


% \cite{chenbehavior}
% \cite{joo2022flexible}

%\todo[inline]{Distributed vs non-distributed, communication vs computational complexity}
%\todo[inline]{Find reference for increased communication needs when distributing MPC}
% Do-mpc, seperating hyperplane


%\todo[inline]{We kind of take a decoupled planning approach. Providing conflict-rich "plans" which are tackled locally.}
